GALA: Generating Animatable Layered Assets from a Single Scan

We present GALA, a framework that takes as input a single-layer clothed 3D human mesh and decomposes it into complete multi-layered 3D assets. The outputs can then be combined with other assets to create novel clothed human avatars with any pose. Existing reconstruction approaches often treat clothed humans as a single-layer of geometry and overlook the inherent compositionality of humans with hairstyles, clothing, and accessories, thereby limiting the utility of the meshes for downstream applications. Decomposing a single-layer mesh into separate layers is a challenging task because it requires the synthesis of plausible geometry and texture for the severely occluded regions. Moreover, even with successful decomposition, meshes are not normalized in terms of poses and body shapes, failing coherent composition with novel identities and poses. To address these challenges, we propose to leverage the general knowledge of a pretrained 2D diffusion model as geometry and appearance prior for humans and other assets. We first separate the input mesh using the 3D surface segmentation extracted from multi-view 2D segmentations. Then we synthesize the missing geometry of different layers in both posed and canonical spaces using a novel pose-guided Score Distillation Sampling (SDS) loss. Once we complete inpainting high-fidelity 3D geometry, we also apply the same SDS loss to its texture to obtain the complete appearance including the initially occluded regions. Through a series of decomposition steps, we obtain multiple layers of 3D assets in a shared canonical space normalized in terms of poses and human shapes, hence supporting effortless composition to novel identities and reanimation with novel poses. Our experiments demonstrate the effectiveness of our approach for decomposition, canonicalization, and composition tasks compared to existing solutions.

==> 03_method_legacy.tex <==


\begin{figure*}[t]
\includegraphics[width=\linewidth]{figs/overview_v5.pdf}
\caption{\textbf{Overview.}}
\label{fig:overview}
\end{figure*}

\section{Overview and Preliminaries}
\label{sec:method}




Our method decomposes a single-layer 3D scan into two complete layers of an object and the rest of the person. To model an object and the remaining human layer, we adopt DMTet~\cite{shen2021dmtet} as our geometric representation. Following previous work~\cite{chen2023fantasia3d}, we first model the geometry of the human and object, and then model the appearance. After initialization (Sec.~\ref{subsection:geometry}), we project 2D segmentation onto a 3D scan, and reconstruct a target asset exclusively in the original space (Sec.~\ref{subsection:reconstructon}). To enable reposing of the layer, we leverage a 2D diffusion prior via SDS loss in canonical space, and synthesize the occluded regions (Sec.~\ref{subsection:canonicalization})
Once we optimize the geometry of the human and the object, we model the appearance using similar SDS losses in the canonical space(Sec.~\ref{subsection:appearance}) such that they can be composed to any humans with any poses. Lastly, we refine the composition of layers by reducing self-penetration (Sec.~\ref{subsection:composition}). 


\subsection{Score Distillation Sampling}
\label{sds}
To synthesize 3D scenes without the need for large-scale 3D datasets, DreamFusion~\cite{poole2023dreamfusion} introduces Score Distillation Sampling (SDS) loss. SDS loss leverages the knowledge of the pretrained 2D diffusion model. Given the target prompt, the loss optimizes over the 3D volume parameterized with $\theta$ using the differentiable renderer $g$, such that the generated image $\mat{x} = g(\theta)$ closely resembles samples from the frozen diffusion model, $\phi$. The gradient of the loss is calculated as,
\begin{equation}
\label{eq:sds}
\begin{split}
    \nabla_{\theta} \mathcal{L}^{SDS}(\mat{x}, \phi) 
    = \mathop{\mathbb{E}} \left[ \omega(t)(\hat{\epsilon_{\phi}}(\mat{x}_t; c, t) - \epsilon) \frac{\partial \mat{x}}{\partial \theta} \right],
\end{split}
\end{equation}
where $c$ denotes text condition and $t$ is the noise level. $\mat{x}_t$ denotes the noised image, $\hat{\epsilon_{\phi}}(\mat{x}_t; c, t)$ represent the noise prediction for the sampled noise $\epsilon$, and $\omega(t)$ is the weighting function. 

\subsection{Deep Marching Tetrahedra}
\label{dmtet}
Deep Marching Tetrahedra~\cite{shen2021dmtet} (DMTet) is a implicit-explicit hybrid 3D representation. It employs a deformable tetrahedral grid denoted as $(\mathbf{X}_{T}, T)$, where $X_T = { \{ \mathbf{x}_i \} }_{i=1\cdots N_{X}}$ represents the grid's 3D vertices $\mathbf{x}_i \in \mathbb{R}^3$ and $T  = { \{ \mathbf{T}_i\} }_{i=1\cdots N_{T}}$ defines the tetrahedral structure, where a tetrahedron ${\mathbf{T}_i}$ contains four vertices in $X_{T}$.
For each vertex $\mathbf{x}_i \in \mathbf{X}_{T}$,
DMTet predicts the signed distance value $s(\mathbf{x}_i)$ from the surface and a position offset $\Delta \mathbf{x}_i$ of each vertex.
We can extract a triangular mesh from the implicit field using the differentiable Marching Tetrahedral (MT) layer.
Since the pipeline is fully differentiable, losses defined explicitly on the surface mesh can be used for optimizing the surface geometry represented by DMTet. 



\section{Method}
\label{sec:method}
\subsection{Representation and Initialization}
\label{subsection:geometry}
We model the geometry of the human and object in separate canonical spaces using DMTet. For a given tetrahedral grid $(X_{T_h}, T_h)$ for the human and $(X_{T_o}, T_o)$ for the object, we utilize MLP networks $\bm{\Psi}_h$ and $\bm{\Psi}_o$ to predict the signed distance value and the deformation offset of every node of the grids. Using the predicted signed distance and offset, the canonical human mesh, $\mesh{M}^c_h=(\mesh{V}^c_h, \mesh{F}_h)$, and the canonical object mesh, $\mesh{M}^c_o=(\mesh{V}^c_o, \mesh{F}_o)$, can be extracted from each grid via a differentiable MT layer.
To obtain a posed mesh, we transform every vertex of the reconstructed mesh via forward linear blend skinning, utilizing the skinning weights of the nearest neighbor vertex of the canonical SMPL-X mesh~\cite{pavlakos2019smplx}. Formally, a vertex $\vec{v}^c \in \mesh{V}^c_h \cup \mesh{V}^c_o$ in canonical space is transferred into posed space with,
\begin{align}
\label{eq:warp}
    \bar{\vec{v}}^p =(\sum_{i=1}^{n_b} w_i \cdot \mat{T}_i(\vec{\beta}, \vec{\theta}))
    \cdot \begin{bmatrix} \mat{I} & \mathcal{B}(\vec{\beta}, \vec{\theta}, \vec{\psi}) \\ 0 & 1 \end{bmatrix} \cdot \bar{\vec{v}}^c,
\end{align}
where $\bar{\vec{v}}^p, \bar{\vec{v}}^c$ are homogeneous coordinates of $\vec{v}^p, \vec{v}^c$ respectively, $n_b$ is the number of bones, $w_i$ is the blend skinning weight of the bone $i$, and $\mat{T}_i(\vec{\beta}, \vec{\theta})\in \mathbb{R}^{4 \times 4}$ is the transformation of the bone $i$ in SMPL-X model given shape parameter $\vec{\beta}\in \mathbb{R}^{10}$ and pose parameter $\vec{\theta} \in \mathbb{R}^{55 \times 3}$. Blend shapes $\mathcal{B}(\vec{\beta}, \vec{\theta}, \vec{\psi})$ are the summation of identity blend shapes, pose blend shapes, and the expression blend shapes, where $\vec{\psi}\in \mathbb{R}^{10}$ is the expression parameter. By transforming all vertices, we get the posed human mesh, $\mesh{M}^p_h=(\mesh{V}^p_h, \mesh{F}_h)$, and the posed object mesh, $\mesh{M}^p_o=(\mesh{V}^p_o, \mesh{F}_o)$.

We initialize the canonical spaces using the canonical SMPL-X geometry,  $\mesh{M}^c_{\text{smpl}}$. We sample points $p \in \mathbb{R}^3$ that are near the surface of $\mesh{M}^c_{\text{smpl}}$ and are uniformly spread in the 3D canonical space and compute the signed distance values, $SDF(p)$, to $\mesh{M}^c_{\text{smpl}}$. 
We employ the following loss functions to guide the initialization of each space.
\begin{gather}
\label{eq:init}
    \mathcal{L}^{init}_{h} = \lVert s(p; \psi_h) - SDF(p) \rVert^2_2 \\
    \mathcal{L}^{init}_{o} = \lVert s(p; \psi_o) - SDF(p) \rVert^2_2
\end{gather}
To this end, we perform the decomposition by minimizing the following total loss, $\mathcal{L}_{geo}$:
\begin{align}
\label{loss_geo}
    \mathcal{L}_{geo} &= \lambda^{rec}_{h}\mathcal{L}^{rec}_{h} + \lambda^{rec}_{o}\mathcal{L}^{rec}_{o} \\ \nonumber
    &+ \lambda^{SDS}_{h}\mathcal{L}^{SDS}_{h} + \lambda^{SDS}_{o}\mathcal{L}^{SDS}_{o} + \lambda^{seg}_{c}\mathcal{L}^{seg}_{c}.
\end{align}







\subsection{Decomposed Reconstruction}
\label{subsection:reconstructon}
To decouple the geometry of the human and object, we employ the 3D surface segmentation of the target object. Specifically, we rasterize the scan from multiple viewpoints and perform binary segmentation in 2D, distinguishing the target object from other elements using an off-the-shelf open-vocabulary segmentation tool~\cite{kirillov2023sam}. Utilizing the pixel-to-face correspondence established during the rasterization process, we cast votes for each face of the mesh to determine whether it belongs to the specified object or not. Consequently, the given input mesh in posed space, denoted as $\mesh{M}^{gt}$, is partitioned into two incomplete surface meshes: the object mesh, $\mesh{M}^{gt}_o$, and the remaining human figure mesh, $\mesh{M}^{gt}_h$.

To preserve the identity of visible regions of the input scan, we employ rendering-based reconstruction losses in the observation space. Using a differentiable rasterizer $\mathcal{R}$ and a sampled camera $k$, we render masks $\mat{M}$ and normal maps $\mat{N}$ of the generated posed meshes $\mesh{M}^p_h$ and $\mesh{M}^p_o$.
\begin{align}
\label{eq:render_recon}
\mat{M}^p_h, \mat{N}^p_h &= \mathcal{R}(\mesh{M}^p_h, \vec{k}) \\
\mat{M}^p_o, \mat{N}^p_o &= \mathcal{R}(\mesh{M}^p_o, \vec{k})
\end{align}
While rendering the mask and normal map of the input mesh, we additionally render segmentation masks, $\mat{S}^{gt}_h$ for the human and $\mat{S}^{gt}_o$ for the object, using the achieved 3D surface segmentation.
\begin{align}
\label{eq:render_recon}
\mat{M}^{gt}, \mat{N}^{gt}, \mat{S}^{gt}_h, \mat{S}^{gt}_o = \mathcal{R}(\mesh{M}^{gt}, \vec{k})
\end{align}
The losses for reconstruction are as follows,
\begin{align}
\label{eq:recon}
\mathcal{L}^{rec}_{h} &= \lVert \mat{N}^p_h \odot \mat{S}^{gt}_h - \mat{N}^{gt} \odot \mat{S}^{gt}_h\rVert^2_2, \\
\mathcal{L}^{rec}_{o} &= \lVert \mat{N}^p_o \odot \mat{S}^{gt}_o - \mat{N}^{gt} \odot \mat{S}^{gt}_o\rVert^2_2
                        + \lVert \mat{M}^p_o - \mat{M}^{gt} \odot \mat{S}^{gt}_o \rVert^2_2.
\end{align}
We employ an additional mask loss to regularize the shape in the posed space.
Furthermore, to capture the intricate details of the human face and hands, we render close-up views of these regions using the posed SMPL-X information and apply the same reconstruction losses.

\begin{figure}[t]
\includegraphics[width=1.0\columnwidth]{figs/cano_w_sds_v3.pdf}
\caption{\textbf{Single scan canonicalization via SDS loss.} Applying our pose-guided SDS loss in the canonical space enables the single scan canonicalization.}
\label{fig:cano_w_sds}
\end{figure}

\subsection{Canonicalization and Synthesis}
\label{subsection:canonicalization}
\begin{itemize}
\end{itemize}
\paragraph{Single Scan Canonicalization}

When the reconstruction loss is applied in the observation space through forward transformation, it is inevitable to have undesired artifacts in the modeled canonical shape as shown in Fig.\ref{fig:cano_w_sds}. This issue arises because multiple points in canonical space can be mapped to a single point in posed space. Hence, previous approaches~\cite{chen2021snarf, Weng_2022_CVPR} rely on having multiple scans or images of a single identity in various poses to model the plausible canonical shape of the identity. To enable plausible canonicalization even when only a single posed scan is available, we propose to leverage the knowledge of 2D diffusion prior of canonicalized human shapes. Specifically, we apply our pose-guided SDS loss w.r.t $\psi_h$ as,
\begin{equation}
\label{eq:sds_hum}
\begin{split}
    \mathcal{L}^{SDS}_h &= \nabla_{\psi_h} \mathcal{L}^{SDS}_h(\tilde{\mat{N}^c_h}, \phi) \\
    &= \mathop{\mathbb{E}} [\omega(t)(\hat{\epsilon_{\phi}}(z_t^{\tilde{\mat{N}^c_h}}; c_{text}, c_{pose}, t) - \epsilon) \frac{\partial \tilde{\mat{N}^c_h}}{\partial \psi_h} \frac{\partial z_t^{\tilde{\mat{N}^c_h}}}{\partial \tilde{\mat{N}^c_h}}],
\end{split}
\end{equation}
where $\tilde{\mat{N}^c_h}$ represents the concatenation of the rendered normal map $\mat{N}^c_h$ and the mask $\mat{M}^c_h$ of the generated canonical human mesh, $\mesh{M}^c_h$, following Fantasia3D~\cite{chen2023fantasia3d}. $\phi$ denotes the parameters of the pretrained Stable Diffusion model~\cite{rombach2022latent}, $c_{text}$ represents the positive and negative text prompts, and $c_{pose}$ is the pose condition injected via OpenPose~\cite{cao2019openpose} ControlNet~\cite{zhang2023controlnet}. $t$ denotes the time step and $\omega(t)$ denotes the weighting function defined by the scheduler of the diffusion model. Remarkably, the utilization of our pose-guided SDS loss in canonical space along with the reconstruction loss of Eq.\ref{eq:recon} in posed space, effectively eliminates implausible correspondences between canonical space and posed space, leading to plausible canonicalization without artifacts. To further discard the artifacts tightly attached to the human torso, we also apply our pose-guided SDS loss in pre-defined poses, in addition to the original canonical pose.



Since it is more natural for clothing to be worn by humans rather than floating in the air on its own, we apply our pose-guided SDS loss to the canonical composition mesh, denoted as $\mesh{M}_c^c$, to model the canonical shape of the object. $\mesh{M}_c^c$ is the merged output of the canonical human mesh, $\mesh{M}^c_h$, and the canonical object mesh, $\mesh{M}^c_o$, by concatenating their vertices and faces. By employing SDS loss in the composition space, the underlying human mesh and the pose condition effectively guide the canonicalization of the human with the object, successfully eliminating the undesired artifacts of the canonical object mesh. Note that we disable the backpropagation of gradients to the human mesh from the SDS loss in composition space to enable the precise canonicalization of the object. The pose-guided SDS loss w.r.t $\psi_o$ is,
\begin{equation}
\label{eq:sds_obj}
\begin{split}
    \mathcal{L}^{SDS}_o &= \nabla_{\psi_o} \mathcal{L}^{SDS}_o(\tilde{\mat{N}^c_c}, \phi) \\
    &= \mathop{\mathbb{E}} [\omega(t)(\hat{\epsilon_{\phi}}(z_t^{\tilde{\mat{N}^c_c}}; c_{text}, c_{pose}, t) - \epsilon) \frac{\partial \tilde{\mat{N}^c_c}}{\partial \psi_o} \frac{\partial z_t^{\tilde{\mat{N}^c_c}}}{\partial \tilde{\mat{N}^c_c}}],
\end{split}
\end{equation}
where $\tilde{\mat{N}^c_c}$ is the concatenation of the rendered normal map $\mat{N}^c_c$ and the mask $\mat{M}^c_c$ of the generated canonical composition mesh, $\mesh{M}^c_c$. Other notations are identical to the ones used in Eq.~\ref{eq:sds_hum}.


\begin{figure}[t]
\includegraphics[width=1.0\columnwidth, trim={1cm 0cm 0.5cm 0.0cm}]{figs/seg_sds_v3.pdf}
\caption{\textbf{Decomposition and Synthesis.} We decompose humans and objects using 3D segmentation lifted from 2D and simultaneously synthesize plausible geometry of the missing regions using SDS loss.}
\label{fig:sds_geo}
\end{figure}

\paragraph{Synthesizing Non-visible Parts}
While separating and canonicalizing the given mesh, we also aim to generate the missing regions resulting from the decomposition process. Moreover, we intend to produce the self-occluded regions of the posed scan to prevent the presence of holes when transformed into different poses. Hence, we again make use of the SDS losses described in  Eq.~\ref{eq:sds_hum} and  Eq.~\ref{eq:sds_obj}. To assure the quality of the generated geometry in the pose of the input mesh, we apply the SDS loss using the renderings of $\mesh{M}^p_h$ and $\mesh{M}^p_c$.

To focus on the synthesis of regions where the human and object initially interacted, we additionally zoom in on these areas by utilizing the bounding box information of the canonicalized object mesh. Furthermore, we have observed that when the hands of the ground-truth mesh are not visible, for instance, when the hands are concealed in pockets or when gloves are worn, utilizing SDS loss alone is not enough for synthesizing high-quality hands. Hence, inspired by previous work~\cite{xiu2023econ, huang2024tech}, we replace the hands of the human with the hands of the SMPL-X after the optimization process.

\paragraph{Segmentation Loss}

In addition to the SDS losses, we incorporate a segmentation loss to further regularize the geometry of each space. Specifically, we assign one-hot encoded vector attributes $[1, 0]$ and $[0, 1]$, respectively to every face of $\mesh{M}^p_h$ and $\mesh{M}^p_o$, and rasterize both meshes together to get the segmentation mask, $\mat{S}^p_c$ of the generated posed composition mesh, $\mesh{M}^p_c$. We minimize the difference between $\mat{S}^p_c$ and the concatenation of rendered ground-truth segmentation masks, $\mat{S}^{gt}_h$ and $\mat{S}^{gt}_o$, with the following loss.
\begin{align}
\label{eq:segmentation}
\mathcal{L}^{seg}_{c} &= \lVert \mat{S}^p_c  - (\mat{S}^{gt}_h \oplus \mat{S}^{gt}_o) \rVert^2_2
\end{align}



\begin{figure}[t]
\includegraphics[width=1.0\columnwidth]{figs/sds_tex_v2.pdf}
\caption{\textbf{Texture Generation.} Applying SDS loss in canonical space generates texture for regions occluded by objects along with self-occluded regions.}
\label{fig:sds_tex}
\end{figure}

\subsection{Appearance Modeling}
\label{subsection:appearance}
\paragraph{Representation and Reconstruction.}
Given the extracted canonical human mesh, $\mesh{M}^c_h$, and canonical object mesh, $\mesh{M}^c_o$, we model the appearance of each mesh using the vertex colors. We employ MLP networks $\bm{\Gamma}_h$ and $\bm{\Gamma}_o$ to predict the albedo of every vertex. Similar to Sec.~\ref{subsection:reconstructon}, we utilize the 3D surface segmentation to initially color the visible regions of the ground truth mesh. Specifically, we render RGB images, denoted $\mat{I}_h^p$ and $\mat{I}_o^p$, along with the masks and segmentation masks using the differentiable rasterizer, and optimize the following losses. 
\begin{align}
\label{eq:recon_tex}
\mathcal{L}^{rec}_{h_{tex}} &= \lVert \mat{I}^p_h \odot \mat{S}^{gt}_h - \mat{I}^{gt} \odot \mat{S}^{gt}_h\rVert^2_2, \\
\mathcal{L}^{rec}_{o_{tex}} &= \lVert \mat{I}^p_o \odot \mat{S}^{gt}_o - \mat{I}^{gt} \odot \mat{S}^{gt}_o\rVert^2_2.
\end{align}

\paragraph{Generation.}
We generate textures for the generated regions during the geometry optimization stage, again utilizing the pose-guided SDS loss. Since we model the appearance of the canonical mesh, our method allows for the recovery of textures for self-occluded regions of the posed ground-truth mesh. Using the same approach of the geometry optimization stage, we apply the SDS loss in the composition space for the generation of textures of the object. Using a differentiable rasterizer, we render the vertex colors of $\mesh{M}^c_h$ and $\mesh{M}^c_c$ to obtain the RGB images, $\mat{I}^c_h$ and $\mat{I}^c_c$. We optimize the parameters $\gamma_h$ of $\bm{\Gamma}_h$ and $\gamma_o$ of $\bm{\Gamma}_o$ by computing the gradients of following SDS losses:
\begin{equation}
\label{eq:sds_hum_tex}
\begin{split}
    \mathcal{L}^{SDS}_{h_{tex}} &= \nabla_{\gamma_h} \mathcal{L}^{SDS}_{h_{tex}}(\mat{x}^c_h, \phi) \\
    &= \mathop{\mathbb{E}} [\omega(t)(\hat{\epsilon_{\phi}}(z_t^{\mat{x}^c_h}; c_{text}, c_{pose}, t) - \epsilon) \frac{\partial \mat{x}^c_h}{\partial \gamma_h} \frac{\partial z_t^{\mat{x}^c_h}}{\partial \mat{x}^c_h}],
\end{split}
\end{equation}
\begin{equation}
\label{eq:sds_obj_tex}
\begin{split}
    \mathcal{L}^{SDS}_{o_{tex}} &= \nabla_{\gamma_o} \mathcal{L}^{SDS}_{o_{tex}}(\mat{x}^c_c, \phi) \\
    &= \mathop{\mathbb{E}} [\omega(t)(\hat{\epsilon_{\phi}}(z_t^{\mat{x}^c_c}; c_{text}, c_{pose}, t) - \epsilon) \frac{\partial \mat{x}^c_c}{\partial \gamma_o} \frac{\partial z_t^{\mat{x}^c_c}}{\partial \mat{x}^c_c}],
\end{split}
\end{equation}
where $\mat{x}^c_h$ and $\mat{x}^c_c$ represent the encoded outputs of $\mat{I}^c_h$ and $\mat{I}^c_c$, achieved using the pretrained image encoder of the diffusion model. All other notations remain consistent with those used in Eq.~\ref{eq:sds_hum}. The total loss, $\mathcal{L}_{tex}$, for optimizing the texture is defined as,
\begin{align}
\label{loss_tex}
    \mathcal{L}_{tex} &= \lambda^{rec}_{h_{tex}}\mathcal{L}^{rec}_{h_{tex}} + \lambda^{rec}_{o_{tex}}\mathcal{L}^{rec}_{o_{tex}}\nonumber \\ &+ \lambda^{SDS}_{h_{tex}}\mathcal{L}^{SDS}_{h_{tex}} + \lambda^{SDS}_{o_{tex}}\mathcal{L}^{SDS}_{o_{tex}}.
\end{align}


\subsection{Composition}
\label{subsection:composition}


In the case of misalignment after the composition of canonicalized assets, we further refine the output by taking advantage of the fact that the object to be transferred should appear as the outermost layer. Given a canonical human mesh, $\mesh{M}^c_h$, and a canonical object mesh, $\mesh{M}^c_o$, we optimize the vertex positions of $\mesh{M}^c_h$ along their normal directions, $\vec{n}_h$. For each vertex $\vec{v}_h \in \mathcal{V}^c_h$ of $\mesh{M}^c_h$, we find its nearest neighbor vertex $\vec{v}^{nn}_h \in \mathcal{V}^{c'}_o \in \mathcal{V}^c_o$ of $\mesh{M}^c_o$, where $\mathcal{V}^{c'}_o$ denotes the visible vertices among $\mathcal{V}^c_o$ when rasterized from multiple views. We introduce a penalty for cases where $\overrightarrow{\vec{v}_h\vec{v}^{nn}_h}$ and $\vec{n}_h$ are oriented in opposite directions. Similarly, for each vertex $\vec{v}_o \in \mathcal{V}^{c'}_o$, we find its nearest neighbor vertex $\vec{v}^{nn}_o \in \mathcal{V}^c_h$, and penalize when $\overrightarrow{\vec{v}_o\vec{v}^{nn}_o}$ and $\vec{n}_o$ have the same direction, where $\vec{n}_o$ denotes the normals of $\vec{v}_o$. Formally, we minimize the following loss,
\begin{align}
\label{loss_refine}
    \mathcal{L}_{ref} &= - \frac{\overrightarrow{\vec{v}_h\vec{v}^{nn}_h}}{\lVert \overrightarrow{\vec{v}_h\vec{v}^{nn}_h} \rVert} \cdot \vec{n}_h + \frac{\overrightarrow{\vec{v}_o\vec{v}^{nn}_o}}{\lVert \overrightarrow{\vec{v}_o\vec{v}^{nn}_o} \rVert} \cdot \vec{n}_o + \lambda_{dis} \lVert \Delta \vec{v}_h \rVert^2_2,
\end{align}
where the last term regularizes the displacements of $\vec{v}_h$.







